Stability theory of game-theoretic group feature explanations for machine learning models

In this article, we study feature attributions of Machine Learning (ML) models originating from linear game values and coalitional values defined as operators on appropriate functional spaces. The main focus is on random games based on the conditional and marginal expectations. The first part of our work formulates a stability theory for these explanation operators by establishing certain bounds for both marginal and conditional explanations. The differences between the two games are then elucidated, such as showing that the marginal explanations can become discontinuous on some naturally-designed domains, while the conditional explanations remain stable. In the second part of our work, group explanation methodologies are devised based on game values with coalition structure, where the features are grouped based on dependencies. We show analytically that grouping features this way has a stabilizing effect on the marginal operator on both group and individual levels, and allows for the unification of marginal and conditional explanations. Our results are verified in a number of numerical experiments where an information-theoretic measure of dependence is used for grouping.

==> Sec6_Examples_KK.tex <==
\section{ \color{brown}Numerical examples}\label{sec::examples}
{\color{brown}This section contains examples that illustrate the theoretical aspects discussed in \S\ref{sec::obser_inter_expl} and  \S\ref{sec::Group_expl}. In the following computations we replace the deterministic marginal explanations with their empirical analogs, which are evaluated as corresponding game values for the empirical marginal game $\hat{v}^{\ME}$ defined by
\begin{equation}\label{empmarggame}
    \hat{v}^{\ME}(S;x,f, \bar{D}_X) := \frac{1}{|\bar{D}_X|}\sum_{ \tilde{x} \in \bar{D}_X} f(x_S,\tilde{x}_{-S}),
\end{equation}
where $x$ is an observation, $f$ is a model, and $\bar{D}_X=\{\tilde{x}^{(k)}\}_{k=1}^K$ is a background dataset of predictor observations used for averaging. 
}

\subsection{Pedagogical example on instability of marginal explanations}\label{sec::pedag_example}


{\color{brown}
The results of \S \ref{sec::obser_inter_expl} show that marginal explanations viewed as linear operators may not be well-defined or stable in $L^2(P_X)$. Demonstrating the instability numerically is not a trivial task because the space $L^2(P_X)$ of models is much larger than any class of models obtained via training. Nevertheless, we numerically investigate the stability of marginal explanations by training a small collection of different models on the same dataset, or on perturbed datasets, and then compare the differences between the resulting explanations as well as between the predictions of those models.
}


We start with a pedagogical example that showcases the instability of marginal explanations under predictor dependencies. Consider the following data generating model. Let $X=(X_1,X_2,X_3)$ be predictors such that the pair $(X_1,X_2)$ is independent of $X_3$, with the distribution given by 
\begin{equation}\label{ex1_preds_}
\begin{aligned}
Z &   \sim { Unif}(-1,1) \\
X_1 & = Z + \epsilon_1, \quad \epsilon_1 \sim \mathcal{N}(0,0.05),\\
X_2 & = \sqrt{2}\sin( Z (\pi/4)) + \epsilon_2, \quad \epsilon_2 \sim \mathcal{N}(0,0.05),\\
X_3 & \sim { Unif}\big([-1,-0.5] \cup [0.5,1] \big).
\end{aligned}
\end{equation}
The model for the output variable is assumed to be 
\begin{equation}\label{ex1_resp_model_}
Y=f_*(X_1,X_2,X_3)+\epsilon_3=3X_2X_3+\epsilon_3, \quad \epsilon_3\sim {Unif}(-0.05,0.05).
\end{equation}

Note that in the true regressor $f_*$ the variable $X_1$ is a dummy variable (it is not explicitly used). For this reason, the marginal {\color{brown}explanation approach will assign zero attribution to this variable.

By design, the dependencies in predictors allow for the existence of many models from $L^2(P_X)$ that approximate the response variable well but have different representations. {\color{brown} In what follows we demonstrate that the generated explanations differ in such cases where different models with distinct representations approximate the data well.}

}


\begin{figure}
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/resp_train_versus_X1.png}\caption{\footnotesize Predictions vs $X_1$.}\label{fig::ex1_pred_vs_X1}
  \end{subfigure}
    \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/resp_train_versus_X2.png}\caption{\footnotesize Predictions vs $X_2$.}\label{fig::ex1_pred_vs_X2}
  \end{subfigure}   
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/resp_train_versus_X3.png}\caption{\footnotesize Predictions vs $X_3$.}\label{fig::ex1_pred_vs_X3}
  \end{subfigure}     
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_train_output_versus_X1.png}\caption{\footnotesize Explanations $\varphi_1$ vs $X_1$.}\label{fig::ex1_explan_vs_X1}
  \end{subfigure}
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_train_output_versus_X2.png}\caption{\footnotesize Explanatons $\varphi_2$ vs $X_2$.}\label{fig::ex1_explan_vs_X2}
  \end{subfigure}
  \begin{subfigure}[t]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_train_output_versus_X3.png}\caption{\footnotesize Explanatons $\varphi_3$ vs $X_3$.}\label{fig::ex1_explan_vs_X3}
  \end{subfigure}
  \caption{ \color{brown} Predictions and marginal Shapley values for XGBoost ($f_1$) and GBM ($f_2$) models.}\label{fig::ex1_pred_explan} 
\end{figure}



\subsubsection{{\color{brown}Case 1: Two models trained on the same dataset.}}

{\color{brown} In our first experiment, we use a training dataset $D_X^{(train)}$ with $25000$ samples drawn from the data generating model \eqref{ex1_resp_model_} and train two regressors {\color{brown}$f_1$ and $f_2$} using the XGBoost and Gradient Boosting (GBM) machine learning algorithms, respectively. The GBM model was trained using the following parameters: {n\_estimators}=$500$, {min\_samples\_split}=$5$, {subsample}=$1.0$, {learning\_rate}=$0.1$. For the XGBoost model we used: {n\_estimators}=$300$, {max\_depth}=$5$, {subsample}=$1.0$, {learning\_rate}=$0.1$, {alpha}=$10$, {lambda}=$10$.}

Performance metrics for the two models on the training and test datasets, both having 25000 samples, were evaluated. {\color{brown} Specifically, the relative $L^2$-errors are approximately $0.058$ and $0.038$, respectively, with the model norms satisfying $\|f_1\|_{L^2(P_X)} \approx 1.379$, $\|f_2\|_{L^2(P_X)} \approx 1.378$. The estimated relative $L^2$-difference between the two models is $0.065$.}

We next pick $m=1000$ samples at random from the training dataset, constructing the dataset {\color{brown} $D^{(e)}_X$ of predictor observations used for explanation}, and use the two regressors to predict the response variable. Figures \ref{fig::ex1_pred_vs_X1}-\ref{fig::ex1_pred_vs_X2} depict the predicted values {\color{brown} for each model versus predictors $X_1$ and $X_2$, respectively,} where we see that both trained models have similar predictions.

{\color{brown}We then evaluate the marginal explanations of each predictor for the two} models, along each sample {\color{brown}$x \in D^{(e)}_X$}. To accomplish this, we make use of the empirical game $\hat{v}^{\ME}(\cdot,x; f_k,\bar{D}_X)$ defined in \eqref{empmarggame} with a background dataset $\bar{D}_X$ used for averaging, which is constructed by randomly drawing $1000$ samples from the training dataset. {\color{brown} Specifically, we compute the Shapley values $\varphi_i[N,\hat{v}^{\ME}](x)$, where $i \in N=\{1,2,3\}$, for each observation $x \in D^{(e)}_X$ and each model $f_k$, $k \in \{1,2\}$. Figures \ref{fig::ex1_explan_vs_X1}-\ref{fig::ex1_explan_vs_X3} depict the distribution of the marginal explanations for predictors $X_1, X_2, X_3$ for each model}, across the dataset {\color{brown}$D^{(e)}_X$}, where we see that the XGBoost model, due to regularization, treats the first predictor as a dummy variable, while the representation of the GBM model relies heavily on the predictor $X_1$. 


\begin{figure}
  \centering
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_norms_train.png} \caption{\footnotesize Explanation norms.}\label{fig::ex1_norm_expl}
  \end{subfigure}  
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_diff_train.png} \caption{\footnotesize Explanation norms of $f_1-f_2$.}\label{fig::ex1_quant_expl_indiv}
  \end{subfigure}
~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_norms_group_train.png} \caption{\footnotesize Quotient explanation norms.}\label{fig::ex1_quant_expl_group}
  \end{subfigure}
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_diff_group_train.png} \caption{\footnotesize Quotient explanations of $f_1-f_2$.}\label{fig::ex1_quant_expl_group2}
  \end{subfigure}
  \caption{ Global individual and quotient explanations.}\label{fig::ex1_quant_expl}
\end{figure}

\begin{figure}
  \centering
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
      \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_gain_tot_stab_train_abs.png} \caption{\footnotesize Total gain in stability.}\label{fig::ex1_quant_expl_gain_stab_tot}
  \end{subfigure}
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_two_models/shap_gain_stab_train_abs.png} \caption{\footnotesize Gain in stability across groups.}\label{fig::ex1_quant_expl_gain_stab_group}
  \end{subfigure}
  \caption{Gain stability.}\label{fig::ex1_gain_stab}
\end{figure}


{\color{brown} To quantify the global attribution of each predictor, we estimate the $L^2$-norms of the marginal Shapley values for each model, $\beta_i(f_k,\vhat^{\ME}):=\|\varphi_i(X;f_k,\vhat^{\ME})\|_{L^2(\P)}$, $i \in N$, which are depicted in Figure \ref{fig::ex1_norm_expl} and recorded in Table \ref{table::exp1_norms}. The values demonstrate that the features $X_1,X_2$ are utilized differently in each model, suggesting that they have different functional representations.

Recall that by Corollary \ref{corr::cond_operator_cont}$(ii)$ (due to the efficiency property of $\varphi$) the conditional Shapley operator is a linear, bounded operator with norm bounded by one and, hence, the conditional Shapley value satisfies $|\beta(f_1-f_2,\vce)|/\|f_1-f_2\|_{L^2(P_X)} \leq 1$, where $\beta:=(\beta_1,\beta_2,\beta_3)$. This bound ensures that the total distance $|\beta(f_1-f_2,\vce)|$ between these explanations is always smaller than the $L^2(P_X)$-distance between the models, and the same is true for any component and sub-vector of the vector $\beta(f_1-f_2,\vce)$. Meanwhile, in theory, in the presence of dependencies, the bound for the marginal explanations may in general be infinite or significantly larger than one, which depends on the relationship between $P_X$ and $\intP_X$.

To understand the degree of the instability in marginal explanations, we estimate the norm of the difference of the marginal Shapley values for the two models. Given the linearity of the marginal operator, this norm is equal to the norm of the Shapley values for the model difference $\beta_i(f_1-f_2,\vhat^{\ME})=\|\varphi_i(X;f_1-f_2,\hat{v}^{\ME})\|_{L^2(\P)}$, whose estimate is given by
\begin{equation}\label{ex1_shap_diff_}
\beta(f_1-f_2,\vhat^{\ME})=(\beta_1,\beta_2,\beta_3)(f_1-f_2,\vhat^{\ME})\approx (0.181, 0.186, 0.051), \,\, \|f_1-f_2\|_{L^2(P_X)} \approx 0.09.
\end{equation}
Observe that the total distance between marginal explanations $|\beta(f_1-f_2,\vhat^{\ME})|_2=0.265$ is approximately three times larger than the $L^2(P_X)$-distance between models. Moreover, the distances between explanations for features $X_1$ and $X_2$ are also approximately twice that of the models; see Figure \ref{fig::ex1_quant_expl_indiv}.  We also note that the total differences between explanations is significant and constitutes about 20\% of the train models' norm; for comparison see Table \ref{table::exp1_norms}.

To understand the effect of grouping,} we construct quotient marginal explanations of the trained models for each sample {\color{brown}$x \in D^{(e)}_X$}. To accomplish this, we employ the empirical quotient marginal game and generate explanations corresponding to the partition $\cP$ based on dependencies, given by $\mathcal{P}=\{\{1,2\},\{3\}\} = \{S_1,S_2\}$. This is done by evaluating quotient Shapley values {\color{brown}$\varphi_j[M,\hat{v}^{\ME,\cP}](x)$, $j \in M=\{1,2\}$, for each observation $x \in D^{(e)}_X$ and each model $f_k$, $k \in \{1,2\}$. 

We then use these explanations to quantify the global attribution of predictor groups by estimating the norms $\beta^{\cP}_j(f_k,\vhat^{\ME}):=\|\varphi^{\cP}_{S_j}(X;f_k,\vhat^{\ME})\|_{L^2(\P)}$, $j \in M$, which are depicted in Figure \ref{fig::ex1_quant_expl_group} and recorded in Table \ref{table::exp1_norms}. These values indicate that grouping by dependencies yields (on average) similar group explanations regardless of the functional representation.

To assess the level of the instabilities in quotient explanations,  we quantify the difference between quotient explanations and compare it with that of between the models. The $L^2$-distance between marginal quotient explanations is given by $\beta^{\cP}(f_1-f_2,\vhat^{\ME})=(\beta^{\cP}_1,\beta^{\cP}_2)(f_1-f_2,\vhat^{\ME})\approx (0.052, 0.049)$. Figure \ref{fig::ex1_quant_expl_group2} compares these distances with those of the models given in \eqref{ex1_shap_diff_}. As a result of grouping by dependencies, these distances are approximately twice smaller than the distances between the models, unlike the global attributions $\beta_i(f_1-f_2,\vhat^{\ME})$ of individual explanations; for comparison see Table \ref{table::exp1_norms}. Moreover, the total distance between quotient marginal explanations $|\beta^{\cP}(f_1-f_2,\vhat^{\ME})|=0.071$  is strictly smaller than the $L^2(P_X)$-distance between models. Thus, due to grouping, the unit bound in \eqref{effvalbound} is satisfied leading to increased stability in $L^2(P_X)$. Finally, the splitting of explanations across dependent predictors does not occur anymore, as was seen in the GBM model.

To estimate the gain in stability due to grouping, we introduce a method that will be useful when dealing with large datasets and where dependencies are not that obvious. Recall that Corollary \ref{corr::cond_operator_cont}$(ii)$   implies $|\beta(f_1-f_2,\vce)| \leq \|f_1-f_2\|$ while Proposition \ref{lmm::boundquot} implies $|\beta^{\cP}(f_1-f_2,\vce)|\leq\|f_1-f_2\|_{L^2(P_X)}$. Thus, to quantify the total gain in stability for marginal explanations across all features we propose to compare $|\beta(f_1-f_2,\vhat^{\ME})|$ and $|\beta^{\cP}(f_1-f_2,\vhat^{\ME})|$ with $\|f_1-f_2\|_{L^2(P_X)}$, which is accomplished in Figure \ref{fig::ex1_quant_expl_gain_stab_tot}. To quantify the gain in stability across each group in $\cP=\{S_1,S_2\}$, we compare the norm of the sub-vector $\beta_{S_j}(f_1-f_2,\vhat^{\ME})$, measuring the aggregated difference across the group $S_j$, with that of $\beta^{\cP}_j(f_1-f_2,\vhat^{\ME})$.  Figure \ref{fig::ex1_quant_expl_gain_stab_group} illustrates that the differences in aggregated explanations drop significantly after grouping, which showcases the gain in stability. It also illustrates that the unit bound is not satisfied for the aggregated explanations, while it is for the quotient ones.

}


\begin{table}
\begin{center}
\begin{tabular}{|c| c | c | c | c | c | c | c | c |}
 \hline
  & $\|\cdot\|$  & $\beta_1$ & $\beta_2$ & $\beta_3$ & $|\beta|$ & $\beta_1^{\cP}$ & $\beta_2^{\cP}$ & $|\beta^{\cP}|$\\[0.5ex]
 \hline
   $f_1$ & {\color{blue}$1.379$} & $0.026$ & $0.667$ & $0.683$ & {\color{blue}$0.955$}  & $0.682$ & $0.681$ &  {\color{blue}$0.964$} \\ 
 \hline 
 $f_2$ & {\color{blue}$1.378$} & $0.192$ & $0.514$ & $0.685$ & {\color{blue}$0.878$} & $0.683$ & $0.682$  & {\color{blue}$0.965$} \\ 
 \hline
 $f_1-f_2$ & {\color{blue}$0.090$} & $0.181$ & $0.187$ & $0.051$ & {\color{blue}$0.265$} & $0.052$ & $0.049$ & {\color{blue}$0.071$}  \\ 
 \hline
\end{tabular}
\caption{Global marginal Shapley attributions.}\label{table::exp1_norms}
\end{center}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\color{brown}Case 2: Models on perturbed datasets}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{
\color{brown} In our second experiment, we construct five distinct datasets by varying the level of noise in the predictors from the previous subsection, and train five corresponding ML models. We then construct a test dataset as a mixture of the five training sets and use its observations for both explanations and averaging. This experiment demonstrates that the models with similar predictive power on the test dataset, which in turn is close in distribution to the training sets, have widely different explanations. It also illustrates how grouping features based on dependencies rectifies the explanation instabilities. The details of the experiment are provided below.

First, for each $\delta \in \{ \delta_i \}_{i=1}^5=\{0.0, 0.001, 0.0025, 0.005, 0.01\}$, which represents the noise level in predictors, we construct a corresponding dataset $D(\delta)=\{(x_{\delta}^{(k)},y_{\delta}^{(k)})\}_{k=1}^K$, containing $K=25000$ observations sampled from the distribution $(X_{\delta},Y_{\delta})$ where $X_{\delta}$ is given by \eqref{ex1_preds_} with  noise $\epsilon_1,\epsilon_2 \sim \mathcal{N}(0,\delta)$, and $Y_{\delta}$ is constructed using the response model \eqref{ex1_resp_model_}. Then for each $i \in \{1,\dots, 5\}$ an XGBoost regressor $f_i(x)$ is trained on the dataset $D(\delta_i)$, utilizing the same hyperparameters as in the previous experiment.

To compare the explanations of these models, a test dataset $D=\{(x^{(k)},y^{(k)})\}_{k=1}^K$ is constructed by drawing  $K=25000$ samples from the distribution $(X,Y)$ such that $X=\sum_{i=1}^5 1_{\{C=i\}} \cdot X_{\delta_i}$ is a mixture, where $C$ is a random variable satisfying $\P(C=i)=0.2$, and $Y$ is obtained using the response model \eqref{ex1_resp_model_}.

}

Performance metrics for the XGBoost models on the mixture dataset were evaluated. Specifically, the relative $L^2$-errors for the five models are approximately $0.051$, $0.045$, $0.041$, $0.052$ and $0.046$, respectively, {\color{brown} with the norms $\|f_i\|_{L^2(P_{X})}$  of the models recorded in Table \ref{table::exp1b_norms}, which illustrates that all trained models have similar predictive power on the test set.}


{\color{brown}
We next evaluate the $L^2(P_{X})$-distance between the true model $f_*$ and each trained model $f_k$, $k\in\{1,\dots,5\}$. The estimated values of the distances are given by
\begin{equation}\label{ex1_pred_diff_mix_}
\|f_k-f_* \|_{L^2(P_{X})}\approx (0.069,0.062,0.056,0.071,0.064), \quad \|f_* \|_{L^2(P_X)}\approx 1.37,
\end{equation}
and also recorded in Table \ref{table::exp1b_norms}. Thus, the predictions of the trained models on the mixture dataset are close in an $L^2$-sense to those of $f_*$. In particular, this implies that $\{f_k\}_{k=1}^5$ live in an $(L^2,\epsilon)$-Rashomon set of models  about $f_*$ (defined in \S\ref{sec::notation}) with $\epsilon=0.071$, which constitutes about 5\% relative $L^2$-distance.}



\begin{figure}
  \centering
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_train_output_versus_X1.png}\caption{\footnotesize Explanations $\varphi_1$ vs $X_1$.}\label{fig::ex1b_explan_vs_X1}
  \end{subfigure}
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_train_output_versus_X2.png}\caption{\footnotesize Explanations $\varphi_2$ vs $X_2$.}\label{fig::ex1b_explan_vs_X2}
   \end{subfigure}
  ~~\\
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_group_train_output_versus_X1.png}\caption{\footnotesize Explanations $\varphi_{S_1}^{\cP}$ vs $X_1$.}\label{fig::ex1b_quot_explan_vs_X1}
  \end{subfigure}
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_group_train_output_versus_X2.png}\caption{\footnotesize Explanations $\varphi_{S_2}^{\cP}$ vs $X_2$.}\label{fig::ex1b_quot_explan_vs_X2}
  \end{subfigure}
\caption{\footnotesize Individual and quotient marginal explanations.} \label{fig::ex1b_expl_mix}
\end{figure}

\begin{figure}
  \centering
    \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_norms_train.png} \caption{\footnotesize Explanation norms.}\label{fig::ex1b_norm_expl_mix}
  \end{subfigure}  
~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_diff_train.png} \caption{\footnotesize Global explanations of $\Delta f_i$.}\label{fig::ex1b_quant_expl_indiv_mix}
  \end{subfigure}
~~\\
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_norms_group_train.png} \caption{\footnotesize Quotient explanation norms.}\label{fig::ex1b_quant_expl_group}
  \end{subfigure}
~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_diff_group_train.png} \caption{\footnotesize Global quotient explanations of $\Delta f_i$.}\label{fig::ex1b_quant_expl_group2}
  \end{subfigure}
  \caption{ Individual and quotient explanation norms.}\label{fig::ex1b_quant_expl}
\end{figure}

We next pick $m=1000$ samples at random from the mixture dataset, constructing the dataset {\color{brown} $D^{(e)}_{X}$ of predictor observations used for explanations}. Similar to the previous example, we construct marginal explanations of each model to understand the contributions of the predictors, including the true model, for each sample $x \in D_{X}$. We first subsample the predictors from the mixture set and obtain a background dataset $\bar{D}_{X}$ with $1000$ samples. The background dataset is then used to construct the empirical marginal game as in \eqref{empmarggame}. We then evaluate the empirical marginal explanations {\color{brown}$\varphi_i[N,\hat{v}^{\ME}](x)$ for each observation $x \in D_X^{(e)}$ } and each predictor across the six models, the true model and the five XGBoost models.



\begin{figure}
  \centering
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_gain_tot_stab_train_abs.png} \caption{\footnotesize Total gain in stability.}\label{fig::ex1b_quant_expl_totgain_stab_abs_mix}
  \end{subfigure}  
  ~~
  \begin{subfigure}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=\textwidth]{pics/instab_explan_many_datasets/shap_gain_stab_train_abs_2.png} \caption{\footnotesize Gain in stability.}\label{fig::ex1b_quant_expl_gain_stab_abs_mix}
  \end{subfigure}
  \caption{Explanation norms and effect of grouping.}\label{fig::ex1b_gain_stab_mix}
\end{figure}

{\color{brown} Figure \ref{fig::ex1b_explan_vs_X1}-\ref{fig::ex1b_explan_vs_X2} depict the scatterplots of explanations for each model across the dataset $D^{(e)}_{X}$, where we see that explanations differ substantially, indicating that the trained models have different functional representations}. In particular,  $f_1$ treats both predictors $X_1,X_2$ similarly due to the strong dependence between them, while $f_5$ treats the first predictor as a dummy variable which is similar to the model $f_*$. 

{\color{brown}
 To quantify the global attribution of each predictor, we estimate the $L^2$-norms of the marginal Shapley values for each model, $\beta_i(f_k,\vhat^{\ME})=\|\varphi_i(X;f_k,\vhat^{\ME})\|_{L^2(\P)}$, $i \in N$, which are depicted in Figure \ref{fig::ex1b_norm_expl_mix} and recorded in Table \ref{table::exp1b_norms}. These values also demonstrate that the features $X_1,X_2$ are utilized differently across the models.

To understand the degree of the instability in marginal explanations, we estimate the distance between the marginal Shapley values of the reference model $f_*$ and $f_k$ for every $k \in \{1,\dots,5\}${\color{red},} which are equal to the norm of the Shapley values for the model difference $\beta_i(f_i-f_*,\vhat^{\ME})=\|\varphi_i(X;f_i-f_*,\hat{v}^{\ME})\|_{L^2(\P)}$, and then compare with those of the model. Figure \ref{fig::ex1b_quant_expl_indiv_mix}, where $f_k - f_*$ is denoted as $\Delta f_k$, showcases the comparison between the distances of the individual feature explanations and the model distances, again for each trained model. 
}


\begin{table}
\begin{center}
\begin{tabular}{|c| c | c | c | c | c | c | c | c |}
 \hline
  & $\|\cdot\|$  & $\beta_1$ & $\beta_2$ & $\beta_3$ & $|\beta|$ & $\beta_1^{\cP}$ & $\beta_2^{\cP}$ & $|\beta^{\cP}|$\\[0.5ex]
 \hline
   $f_1$ & {\color{blue}$1.370$}  & $0.674$ & $0.000$  & $0.675$ & 
           {\color{blue}$0.954$}  & $0.674$ & $0.675$  & {\color{blue}$0.954$} \\ 
 \hline 
 $f_2$   & {\color{blue}$1.375$}  & $0.334$ & $0.385$  & $0.685$ & 
           {\color{blue}$0.854$}  & $0.681$ & $0.683$  & {\color{blue}$0.964$} \\ 
 \hline 
 $f_3$   & {\color{blue}$1.374$}  & $0.285$ & $0.461$  & $0.682$ & 
           {\color{blue}$0.871$}  & $0.680$ & $0.681$  & {\color{blue}$0.962$} \\ 
 \hline 
 $f_4$   & {\color{blue}$1.375$}  & $0.214$ & $0.228$ & $0.040$ & 
           {\color{blue}$0.315$}  & $0.679$ & $0.681$ & {\color{blue}$0.962$} \\ 
 \hline 
 $f_5$   & {\color{blue}$1.374$}  & $0.068$ & $0.627$  & $0.677$ & 
           {\color{blue}$0.925$}  & $0.678$ & $0.680$  & {\color{blue}$0.960$} \\ 
 \hline
 $f_*$   & {\color{blue}$1.380$}  & $0.000$ & $0.682$  & $0.682$ & 
           {\color{blue}$0.965$}  & $0.682$ & $0.683$  & {\color{blue}$0.965$} \\ 
 \hline
 $f_1-f_*$ & {\color{blue}$0.069$} & $0.674$ & $0.682$ & $0.036$ &
             {\color{blue}$0.960$} & $0.038$ & $0.036$ & {\color{blue}$0.052$}  \\ 
 \hline
 $f_2-f_*$ & {\color{blue}$0.062$} & $0.334$ & $0.336$ & $0.035$ & 
             {\color{blue}$0.475$} & $0.032$ & $0.028$ & {\color{blue}$0.042$}  \\ 
 \hline
 $f_3-f_*$ & {\color{blue}$0.056$} & $0.284$ & $0.288$ & $0.033$ & 
             {\color{blue}$0.406$} & $0.029$ & $0.026$ & {\color{blue}$0.039$}  \\ 
 \hline
 $f_4-f_*$ & {\color{blue}$0.071$} & $0.214$ & $0.228$ & $0.041$ & 
             {\color{blue}$0.315$} & $0.044$ & $0.029$ & {\color{blue}$0.053$}  \\ 
 \hline
 $f_5-f_*$ & {\color{blue}$0.064$} & $0.067$ & $0.075$ & $0.029$ & 
             {\color{blue}$0.104$} & $0.027$ & $0.026$ & {\color{blue}$0.037$}  \\ 
 \hline
\end{tabular}
\caption{ Global marginal Shapley attributions.}\label{table::exp1b_norms}
\end{center}
\end{table}
As in the previous experiment, we contrast the unit operator bound in \eqref{effvalbound} for conditional explanations in relation to the change in empirical marginal explanations with respect to the $L^2(P_X)$-distance between models. Specifically, the ratio of the  marginal explanation distance to the distance between models varies from approximately $1$ to $10$; see Figure \ref{fig::ex1b_quant_expl_indiv_mix}. Note that the differences between explanations are significant and for some models constitute about 50\% of the {\color{brown}true} model's norm. {\color{brown} Observe also, that the total distances between the vectors of global marginal explanations satisfy $\{|\beta(f_i-f_*,\vhat^{\ME})|\}_{i=1}^5=\{0.960,0.475,0.406,0.315,0.104\}$ and are approximately two-to-fourteen times larger than the $L^2(P_X)$-distance between models; see Figure \ref{fig::ex1b_quant_expl_gain_stab_abs_mix}. We note that the total distance between explanations is significant and, in particular, for the model $f_1$ it constitutes about 60\% of the trained models' norm; see Table \ref{table::exp1b_norms}.} 


We next construct the quotient marginal explanations for each model. Figure \ref{fig::ex1b_quot_explan_vs_X1}-\ref{fig::ex1b_quot_explan_vs_X2} depict the scatterplots of quotient explanations for each model across the dataset $D_{X}$, where we see that the explanations between the models are similar.

To quantify the difference between quotient explanations, we estimate $L^2(P_X)$-norms of quotient marginal explanations and the $L^2(P_X)$-distances between marginal quotient explanations {\color{brown} for the partition $\cP=\{\{1,2\},\{3\}\}=\{S_1,S_2\}$}, {\color{brown} denoted by $\beta^{\cP}_j(f_i,\vhat^{\ME})$ and $\beta^{\cP}_j(f_i-f_*,\vhat^{\ME})$, $j \in \{1,2\}$, respectively. Figure \ref{fig::ex1b_quant_expl_group} illustrates the former and Figure \ref{fig::ex1b_quant_expl_group2} compares the latter with distances between the models given in \eqref{ex1_pred_diff_mix_}.} As in the previous case, again due to grouping, we see that these distances are approximately twice smaller than the distances between the models compared to individual explanations, showcasing the consistency with the bound for conditional explanations. The contrast between Figures \ref{fig::ex1b_quant_expl_indiv_mix} and \ref{fig::ex1b_quant_expl_group2}, as before, demonstrates that grouping by dependencies reduces the splitting of {\color{brown}explanations} across dependent predictors.


To quantify the gain in stability due to grouping, we apply the approach outlined in the previous experiment. {\color{brown} Specifically, we compare the norm of explanation vectors $|\beta(f_i-f_*,\vhat^{\ME})|$ and $|\beta^{\cP}(f_i-f_*,\vhat^{\ME})|$ to quantify the total gain in stability (across all features simultaneously), which is depicted in Figure \ref{fig::ex1b_quant_expl_totgain_stab_abs_mix}. We also compare the norms of the quotient explanations' differences for each $j\in M$ with the length of corresponding subvectors $|\beta_{S_j}(f_i-f_*,\vhat^{\ME})|$.} Figure \ref{fig::ex1b_quant_expl_gain_stab_abs_mix} illustrates that the differences in aggregated individual explanations drop significantly after grouping, and well below the $L^2(P_X)$-norm of the model difference, which showcases the gain in stability {\color{brown} across each group}. 


{
\color{brown}
\subsection{Application to public datasets}

In this section, we apply the group explanation techniques to public datasets. % \begin{itemize}
% \item \href{https://archive.ics.uci.edu/dataset/350/default+of+credit+card+clients}{Default of Credit Card Clients dataset} \cite{default_credit_dataset} a classification dataset where .
% \item \href{https://archive.ics.uci.edu/ml/datasets/superconductivty+data}{The Superconductivity dataset} \cite{superconductivty_dataset}: 
% a regression dataset where the 
% superconductivity critical temperature should be predicted based on $81$ features extracted from the superconductor’s chemical formula. The original dataset has $21263$ instances. % We randomly split it into training and test sets in $90:10$ proportions.
% \end{itemize}
We start our investigation with the Default of Credit Card Clients dataset \cite{default_credit_dataset} from the UCI Machine Learning Repository. This dataset {\color{blue}contains $30000$ instances,} 23 features and a dependent binary variable $Y$ that indicates if an individual defaulted on a payment, where the default is denoted by $Y=1$. {\color{blue}The protected attributes `sex', `marriage', and `age' were removed in order to be consistent with regulatory practices}. The remaining twenty predictors were used for model training, where we use the training dataset $D_{train}$ with $27000$ samples to build a classification score $p_*(x)=\widehat{\PP}(Y=1|X=x)$ using {\color{blue}the CatBoost algorithm}, whose corresponding  population minimizer is defined by $f_*(x)=\logit(p_*(x))$. For training we use the following parameters: iterations=$200$, min\_data\_in\_leaf=$5$, depth=$5$, subsample=$0.8$, and learning\_rate=$0.1$.

Performance metrics for the model on the trained dataset, and test dataset with $3000$ samples, were evaluated. Specifically, the mean logloss on the train and test set is approximately $0.40$ and $0.41$ respectively, and the AUC is $0.82$ and $0.80$ respectively.


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_ranking/hierclust_MIC_average_.png}
        % \caption{\footnotesize MIC-based hierarchical clustering with GA linkage. \vspace{5pt}}
        % \label{fig::MIC_tree_credit}
    \end{subfigure}
    \caption{\footnotesize \color{brown} MIC-based hierarchical clustering for the Default of Credit Card Clients dataset.}\label{fig::MIC_tree_credit_}
\end{figure}

{\color{blue}To assess the dependencies}, we build a dendrogram based on the MIC-metric and investigate the level of dependence that exists among the twenty predictors. As seen in Figure \ref{fig::MIC_tree_credit_}, the dependencies are not as extreme as the {\color{blue}ones} designed in the synthetic dataset of \S\ref{sec::pedag_example}. There we were able to showcase {\color{blue}the} drastic Rashomon effect because the models we designed {\color{blue}\sout{(intentionally)}} {\color{blue}exhibit stronger dependencies between predictors}. In particular, Figures \ref{fig::ex1_norm_expl} and \ref{fig::ex1b_norm_expl_mix} in  \S\ref{sec::pedag_example} depicting the norms of marginal explanations for each predictor illustrate the ``importance'' of these predictors for each {\color{blue}model}. Some models view the first two predictors as being similar, while {\color{blue}\sout{some}} others put more emphasis on one of them. As we will see, the Rashomon effect is still present {\color{blue}in} the models trained on the Default of Credit Clients dataset and grouping leads to {\color{blue}higher} stability, but not as drastically in light of the lack of strong dependencies.

In what follows, we will compute the empirical marginal Owen values $\{Ow(x;\empvme, \cP, f_*)\}_{i=1}^{20}$ defined in \eqref{BzOw} for different partitions $\cP$ obtained by thresholding the tree. Recall from \S\ref{sec::ExTree} that the tree can be viewed as a coalescent process parameterized by $\alpha=1-\MICe$. This yields a sequence of nested partitions $\{\cP^{(k)}\}_{k=0}^{19}$, with $\cP^{(k)}$ corresponding to the $k$-th coalescent, and having $(20-k)$ groups of predictors. 

In \S\ref{sec::obser_inter_expl}, we discussed two phenomena associated with efficient game values under dependencies: 1) the energy of the model (i.e. its norm squared) {\color{blue}dissipating among explanations of dependent predictors} (see \eqref{energyineq}, and Examples \ref{ex::energycons}, \ref{ex::energy_dissip_dep} and \ref{ex::energy_dissip_int}), and 2) similar models that approximate the same data can have very different marginal explanations (see Examples \ref{ex::marg_illposed} and \ref{ex::marg_instab}, and Theorem \ref{thm::margoperatorunbound}) in view of the Rashomon effect. As we will see in the context of marginal explanations, both phenomena may take place simultaneously. In what follows, we will explore these issues by first investigating the issue of {\color{blue}energy} splits and then discussing the Rashomon effect.



\subsubsection{Ranking and energy splitting of explanations}\label{sec::num_ranking}

Here, we consider partition $\cP^{(8)}=\cP_{0.49}$, that can be obtained by thresholding the {\color{blue}dendrogram} at $\alpha=0.49$. This partition contains the following groups: \{PAY\_0,PAY\_2\}, \{PAY\_3,PAY\_4\}, \{PAY\_5,PAY\_6\}, \{BILL\_AMT1,\dots,BILL\_AMT6\}, and the rest are singletons; see Figure \ref{fig::MIC_tree_credit_}. 


We then compute the (global) empirical marginal Owen explanations of the population minimizer $f_*(x)$, the values $\beta_i(f_*,\vhat^{\ME})=\|Ow_i(X;f_*,\cP^{(8)},\vhat^{\ME})\|_{L^2(\P)}$, $i \in N$, which are depicted in Figure \ref{fig::expl_norms_credit_}.   To accomplish this, we use the empirical game defined in \eqref{empmarggame} with a background dataset $\bar{D}_X:=D_{train}$. To compute the explanations of the population minimizer, given the dimensions of the background dataset, we use the fast, exact algorithm introduced in Filom et al. \cite{FilomTBMarg}, which is designed specifically for the computation of empirical marginal coalitional values of CatBoost ensembles.


% {\color{magenta} We note that the complexity of these explanations is $O(2^{12}\cdot |\bar{D}_X|)$; compare with $2^{20} \cdot |\bar{D}_X|$ for the Shapley value.} 

We then compute the sums of explanations over each group to obtain the global contributions of the groups themselves, the values $\beta_j^{\cP^{(8)}}(f_*,\vhat^{\ME})=\|Ow_{S_j}(X;f_*,\cP^{(8)},\vhat^{\ME})\|_{L^2(\P)}$, $S_j \in \cP^{(8)}$, which are depicted in Figure \ref{fig::expl_norms_credit_}. Recall from \S\ref{sec::qp_prop} that the group sums are equal to the quotient Shapley values in view of {\color{blue}\sout{the}} \eqref{quotientgame} {\color{blue}\sout{property}}. Since groups are not fully independent, the quotient marginal Shapley values are only crude approximants of the conditional ones. 


To observe the splits, it is sufficient to compare the contributions of highly dependent predictors that form the coalition with that of the coalition itself as well as with contributions of independent (or almost independent) predictors that form singletons and whose marginal explanations, according to Proposition \ref{prop::unifcoalexpl}, are equal to (or approximate well) the corresponding conditional ones.


The splits are prominent in Figure \ref{fig::expl_norms_credit_} which presents the {\color{blue}norms of} contributions of the individual predictors together with the corresponding groups. Observe the energy splitting occurring in the predictor group with BILL\_AMT's and contrast the individual and group explanations with, for example, the explanation of LIMIT\_BAL. When one attempts to rank order predictors based on their contributions, LIMIT\_BAL will be placed higher in the ranking compared to each BILL\_AMT. However, when ranking groups, \{LIMIT\_BAL\}, as a singleton, will be placed lower than the group containing the BILL\_AMT predictors. This clearly indicates the issue {\color{blue}caused by energy splits to rank ordering} based on contributions of individual predictors.

To complete our study, we repeat the same experiment by computing empirical marginal Shapley values and compare them with those of sums of marginal  Shapley values for the model $f_*$; see Figure \ref{fig::expl_norms_shap_credit_}. It can be seen that the global marginal Owen and Shapley explanations are extremely similar. We believe this is due to the fact that $f_*$ is close to `additive' (since $f_*=\beta +\alpha(\sum \mathcal{T}_j)$ where each oblivious tree $\mathcal{T}_j$ is {\color{blue}a} function of at most $5$ variables) and the dependencies between predictors are not very strong. Furthermore, the linearity of the game value implies that Owen and Shapley explanations are linear combinations of explanations for each individual tree. Although the marginal Owen and Shapley values for a given tree in general differ (since a tree is not an additive function), the trees in this model are not very deep and oblivious, which apparently leads to values being very similar.


}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_ranking/expl_norms_model_2_part_8.png}
        % \caption{\footnotesize Explanation norms. \vspace{5pt}}
        % \label{fig::expl_norms_credit}
    \end{subfigure}
    \caption{\footnotesize Global Owen explanation for $\cp^{(8)}=\cP_{0.49}$.}\label{fig::expl_norms_credit_}
\end{figure}




\begin{figure}
    \centering
    \begin{subfigure}[t]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_ranking/expl_norms_shap_vs_sum_shap_model_2_part_8.png}
        % \caption{\footnotesize Explanation norms. \vspace{5pt}}
        % \label{fig::expl_norms_credit}
    \end{subfigure}
    \caption{\footnotesize Global Shapley explanation for $\cP^{(8)}=\cP_{0.49}$.}\label{fig::expl_norms_shap_credit_}
\end{figure}


\subsubsection{Grouping effect on stability}\label{sec::num_stability}

{\color{blue}
In this section, we continue to explore the Rashomon effect by measuring and comparing the stability of explanations before and after grouping {\color{red}on the Default of Credit Card Clients dataset \cite{Yeh2009}}.

To understand how the dependencies between groups affect stability, we design the following experiment. Given the reference model $f_*$ {\color{red}and} the population minimizer described in Section \ref{sec::num_ranking}, we train a series of new models whose predictions are close to {\color{red}those} of $f_*$ by varying the hyperparameters. Specifically, we pick the following parameters at random from the given intervals: iterations $\in [50,300]$, subsample $\in [0.5,1.0]$, depth $\in [2,10]$, learning\_rate $\in[0.025,0.25]$, rsm $\in[0.5,0.1]$, with the rest of the parameters being the same as for $f_*$. We then train a new model $f$ and accept or reject based on the following principle. Given a threshold $\tau \in [0,1]$, we accept the model if it is in the Rashomon ball of {\color{red}\sout{the}} relative radius $\tau$, meaning that $\hat{\E}[|f(X)-f_*(X)|^2] \leq \tau \|f_*\|_{L^2(P_X)}$, otherwise it is rejected; here $\|f_*\|_{L^2(P_X)} \approx 1.84$ which is estimated on the test set, and we choose $\tau = 0.1$. We continue this procedure until we train 20 models $\{f_k\}_{k=1}^{20} $ {\color{red}\sout{that ``live'' in the Rashomon ball centered at $f_*$ of relative (with respect to $f_*$) size $\tau=0.1$}}.

We next consider partitions of features with {\color{red}varying} degrees of dependence, from moderate {\color{red}\sout{level}} to strongly dependent. This task is accomplished by cross-sectioning the partition tree of dependencies for a given dataset at different heights. {\color{red}In this analysis} the partitions considered are $\cP_{0.49}$, $\cP_{0.62}$, $\cP_{0.65}$ and $\cP_{0.77}$, containing $12$, $10$, $9$, and $5$ groups (see Figure \ref{fig::MIC_tree_credit_2}), respectively, with the subscript indicating {\color{red}the} cutoff threshold.

Given these four partitions we evaluate the empirical marginal Owen explanations for each predictor and for each group (via summation) per model. Subsequently, we compute the global explanation of the model difference $\|f_*-f_k\|_{L^2(\P)}$  from individual explanations. Specifically, we first evaluate the explanations $Ow_i (X,f_*-f_k,\empvme,\cP)$  of the model difference $\Delta f_k = f_*-f_k$ and then compute the corresponding norms $\beta_i (f_*-f_k,\cP)={\color{red}\|Ow_i (x,f_*-f_k,\cP)\|_{L^2(\P)}}$, $i \in N$, for each $k\in\{1,\dots,20\}$ and  $\cP \in \{P_{0.49},P_{0.62},P_{0.65},P_{0.77}\}$. We do the same for the group explanations, $\beta_{j}^{\cP} (f_k-f_*,\cP)=\|Ow_{S_j} (X,f_k-f_*,\empvme,\cP)\|_{L^2(\P)}$, $j \in M$.


To contrast the stabilization effect between individual and group explanations, we evaluate the length of the vectors $\beta(f_*-f_k,\cP)=\{\beta_i(f_*-f_k,\cP)\}_{i \in N}$ and $\beta^{\cP}(f_*-f_k,\cP)=\{\beta^{\cP}_{j}(f_*-f_k,\cP)\}_{j \in M}$ and compute the maximum of these quantities across all models $k\in\{1,\dots,20\}$. These are plotted in Figure \ref{fig::Expl_Diff_Tot_Ind_Group_singl} together with the norm of the maximum model difference. As we see in the plot, the total group explanation differences are smaller than the respective total individual {\color{red}ones}, showcasing the gain in stability when considering explanations of groups. Furthermore, as we reach partition $\cP_{0.77}$, observe that the total group explanation difference becomes approximately equal to the norm of the difference of the models, illustrating the alleviation of the Rashomon effect due to weaker dependencies between the groups. Note that in {\color{red}\sout{the second}} Figure \ref{fig::Expl_Diff_Tot_Ind_Group_nosingl} we have removed the energy contributed by {\color{red}\sout{groups containing}} singletons from both individual and group explanation vectors, since these do not have any effect on the norm evaluation between the two.


Given that the dependencies are not very strong in the Default of Credit Clients dataset, as seen in the partition tree in Figure \ref{fig::MIC_tree_credit_2}, note that the Rashomon effect in general is not as prominent as in the synthetic example from \S\ref{sec::pedag_example}, but it is still present. Nevertheless, Figure \ref{fig::Expl_Diff_Tot_Ind_Group_} still portrays this effect and its alleviation when predictor groups are considered based on dependencies.

\begin{table}
\begin{center}
\begin{tabular}{|c| c | c | c | c | c | c | c | c |}
\hline
& $\|f_*\|$ & $\max_k \|\Delta f_k\|$ &  $\max_k|\beta(\Delta f_k,\cP)|$ & $\max_k|\beta^{\cP}(\Delta f_k,\cP)|$\\[0.5ex]
\hline
$\cP_{0.49}$   &$1.839$ & $0.267$ & $0.388$ &  $0.364$  \\ 
 \hline 
 $\cP_{0.62}$  &$1.839$ & $0.267$ & $0.390$  & $0.388$   \\ 
 \hline 
 $\cP_{0.65}$  &$1.839$ & $0.267$ & $0.389$  & $0.340$   \\ 
 \hline 
 $\cP_{0.77}$  &$1.839$ & $0.267$ & $0.386$  & $0.269$   \\ 
 \hline
\end{tabular}
\caption{ Global marginal Owen attributions for Default of Credit Card Clients dataset.}\label{table::exp2a_norms}
\end{center}
\end{table}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_stability/hierclust_MIC_average_.png}
    \end{subfigure}
    \caption{\footnotesize  MIC-based hierarchical clustering for the Default of Credit Card Clients dataset with 4 cutoffs.}\label{fig::MIC_tree_credit_2}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_stability/diff_expl_tot_model_0.png}
        \caption{\footnotesize Norms of explanation differences (with singletons).}\label{fig::Expl_Diff_Tot_Ind_Group_singl}
    \end{subfigure}
    ~~
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/default_credit_stability/diff_expl_tot_nonsingl_model_0.png}
        \caption{\footnotesize Norms of explanation differences (without singletons).}\label{fig::Expl_Diff_Tot_Ind_Group_nosingl}
    \end{subfigure}    
    \caption{\footnotesize Gain in stability, $|\beta|$ versus $|\beta^{\cP}|$. Deafult of Credt Card Clients dataset.}\label{fig::Expl_Diff_Tot_Ind_Group_}
\end{figure}



We next consider the Superconductivity dataset \cite{superconductivty_dataset}, a regression dataset where the superconductivity critical temperature is predicted based on $81$ features extracted from the superconductor’s chemical formula. The original dataset has $21263$ instances. As before, we first construct a hierarchical clustering tree of feature dependencies using the MIC-based metric (see Figure \ref{fig::MIC_tree_superconductivity}) in order to form partitions. The dataset is then randomly split into training and test sets in $90$:$10$ proportions, and we train a (reference) regressor model $f_*(x)=\hat{\E}[Y|X=x]$ using the CatBoost algorithm. For training we use the following parameters: iterations=$300$, min\_data\_in\_leaf=$5$, depth=$8$, subsample=$0.8$, and learning\_rate=$0.1$. {\color{red}KK: Made into one paragraph.}

Performance metrics for the model on the trained and test datasets, the latter with $2126$ samples, were evaluated. Specifically, the mean square error estimate on the training and test sets is approximately $7.70$ and $9.45$ respectively, which constitutes about $16\%$ and $20\%$ of relative error given that the $L^2$-norm estimate of the reference model is $\|f_*\|_{L^2(P_X)} \approx 47.48$ on the test dataset.



Following the above methodology, we train a series of new models whose predictions are close to the predictions of $f_*$. Specifically, we pick the following parameters at random from the given intervals: iterations $ \in [100,500]$, subsample $\in[0.5,1.0]$, depth $\in[4,10]$, learning\_rate $\in[0.025,0.25]$, rsm $\in [0.5,0.1]$, with the rest of the parameters being the same as for $f_*$. We then train a new model $f$ and accept it {\color{red}if it is in the Rashomon ball centered at $f_*$  of relative size $\tau=0.06$, meaning if $\hat{\E}[|f(X)-f_*(X)|^2] \leq \tau \|f_*\|_{L^2(P_X)}$, or reject otherwise. We continue this procedure until we construct 25 models $\{f_k\}_{k=1}^{25}$}.

Similar to the previous dataset, the partitions considered in this analysis are $\cP_{0.3}$, $\cP_{0.4}$, $\cP_{0.5}$, $\cP_{0.56}$, $\cP_{0.60}$ and $\cP_{0.65}$; see Figure \ref{fig::MIC_tree_superconductivity}. Given these six partitions we evaluate, as before, the empirical marginal Owen explanations for each predictor and for each group (via summation) per model and then evaluate the length of their global explanations. These are plotted in Figure \ref{fig::Expl_Diff_Tot_Ind_Group_sc_singl} together with the norm of the maximum model difference. Once again, the total group explanation differences are smaller than the respective total individual {\color{red}ones}, showcasing the gain in stability when considering explanations of groups. Furthermore, as we reach partition $\cP_{0.77}$, observe that the total group explanation difference becomes approximately equal to the norm of the difference of the models, illustrating again the alleviation of the Rashomon effect.

\begin{table}
\begin{center}
\begin{tabular}{|c| c | c | c | c | c | c | c | c |}
\hline
& $\|f_*\|$ & $\max_k \|\Delta f_k\|$ &  $\max_k|\beta(\Delta f_k,\cP)|$ & $\max_k|\beta^{\cP}(\Delta f_k,\cP)|$\\[0.5ex]
\hline
$\cP_{0.3}$   &$47.482$ & $2.808$ & $11.286$  & $7.207$  \\ 
\hline 
$\cP_{0.4}$   &$47.482$ & $2.808$ & $11.269$  & $6.479$  \\ 
\hline 
$\cP_{0.5}$   &$47.482$ & $2.808$ & $11.119$  & $5.018$  \\ 
\hline 
$\cP_{0.55}$  &$47.482$ & $2.808$ & $11.146$  & $4.971$  \\ 
\hline
$\cP_{0.60}$  &$47.482$ & $2.808$ & $11.150$  & $4.054$  \\ 
\hline
$\cP_{0.66}$  &$47.482$ & $2.808$ & $11.167$  & $2.454$  \\ 
\hline
\end{tabular}
\caption{ Global marginal Owen attributions for Superconductivity dataset.}\label{table::exp2b_norms}
\end{center}
\end{table}

We would like to contrast this dataset with the Default of Credit Card Clients dataset. Note that due to the stronger dependencies among the features of the Superconductivity dataset, the Rashomon effect is much more apparent in this case compared to the previous dataset, which also means that the alleviation of the Rashomon effect due to evaluating group explanations is also more striking.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/super_conductivity/hierclust_MIC_average_.png}
    \end{subfigure}
    \caption{\footnotesize \color{blue} MIC-based hierarchical clustering for the Superconductivity dataset with $6$ cutoffs.}\label{fig::MIC_tree_superconductivity}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/super_conductivity/diff_expl_tot_model_0.png}
        \caption{\footnotesize Norms of explanation differences (with singletons).}\label{fig::Expl_Diff_Tot_Ind_Group_sc_singl}
    \end{subfigure}
    ~~
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pics/super_conductivity/diff_expl_tot_nonsingl_model_0.png}
        \caption{\footnotesize Norms of explanation differences (without singletons).}\label{fig::Expl_Diff_Tot_Ind_Group_sc_nosingl}
    \end{subfigure}    
    \caption{\footnotesize Gain in stability, $|\beta|$ versus $|\beta^{\cP}|$. Superconductivity dataset.}\label{fig::Expl_Diff_Tot_Ind_Group_sc}
\end{figure}

}
